Parts2Words: Learning Joint Embedding of Point Clouds and Texts by Bidirectional Matching between Parts and Words

Shape-Text matching is an important task of high-level shape understanding. Current methods mainly represent a 3D shape as multiple 2D rendered views, which obviously can not be understood well due to the structural ambiguity caused by self-occlusion in the limited number of views. To resolve this issue, we directly represent 3D shapes as point clouds, and propose to learn joint embedding of point clouds and texts by bidirectional matching between parts from shapes and words from texts. Specifically, we first segment the point clouds into parts, and then leverage optimal transport method to match parts and words in an optimized feature space, where each part is represented by aggregating features of all points within it and each word is abstracted by its contextual information. We optimize the feature space in order to enlarge the similarities between the paired training samples, while simultaneously maximizing the margin between the unpaired ones. Experiments demonstrate that our method achieves a significant improvement in accuracy over the SOTAs on multi-modal retrieval tasks under the Text2Shape dataset. Codes are available at https://github.com/JLUtangchuan/Parts2Words.

==> sections/figtable/ablationstudy.tex <==
\begin{table*}\centering
\caption{Ablation study results of the proposed model.}
\label{cmp:ablation study}

\vspace{0.1cm}\centering\begin{tabular}{cccccc|ccc|ccc} 
\hline
\multicolumn{6}{c|}{{}} & \multicolumn{3}{c|}{S2T} & \multicolumn{3}{c}{T2S} \\
Backbones & Matching & w/o e2e & w/o semi & w/o color & w/o seg loss & RR@1 & RR@5 & NDCG@5 & RR@1 & RR@5 & NDCG@5 \\
\hline
PN++ & EMD &  &  &  &  & 16.66     & 43.11    & 13.20  & 11.10     & 28.89    & 20.25 \\
PN & CD &  &  &  &  & 18.47     & 45.98    & 14.52    & 11.73     & 32.60    & 22.49    \\
PN & EMD & \checkmark &  &  &  & 16.31    & 43.39    & 12.99    & 10.68    & 29.25    & 20.14   \\ 
PN & EMD &  & \checkmark &  &  & 0.00     & 0.21    & 0.04  & 0.08     & 0.35    & 0.23    \\
PN & EMD &  &  & \checkmark &   & 7.77    & 26.94    & 6.91   & 5.06    & 17.21    & 11.25   \\
PN & EMD &  &  &  & \checkmark  & 11.62    & 29.18    & 8.53   & 7.58    & 21.93    & 14.91   \\
\hline
PN & EMD &  &  &  &  & \textbf{19.38}     & \textbf{47.17}    & \textbf{15.30}  & \textbf{12.72}     & \textbf{32.98}    & \textbf{23.13}\\
\hline
\end{tabular}
\end{table*}
